Automating Cluster Management with Weave

Modern cluster management systems like Kubernetes and Openstack grapple with hard combinatorial optimization problems: load balancing, placement, scheduling, and configuration. Currently, developers tackle these problems by designing custom application-specific algorithms---an approach that is proving unsustainable, as ad-hoc solutions both perform poorly and introduce overwhelming complexity to the system, making it challenging to add important new features. We propose a radically different architecture, where programmers drive cluster management tasks declaratively, using SQL queries over cluster state stored in a relational database. These queries capture in a natural way both constraints on the cluster configuration as well as optimization objectives. When a cluster reconfiguration is required at runtime, our tool, called Weave, synthesizes an encoding of these queries into an optimization model, which it solves using an off-the-shelf solver. We demonstrate Weave's efficacy by powering three production-grade systems with it: a Kubernetes scheduler, a virtual machine management solution, and a distributed transactional datastore. Using Weave, we expressed complex cluster management policies in under 20 lines of SQL, easily added new features to these existing systems, and significantly improved placement quality and convergence times.

==> sections/background.tex <==
\subsection{Specialized solvers}
\label{sec:background}

In this section we briefly overview the constraint solving technology.
Constraint solvers are a class of tools designed to tackle hard combinatorial problems~\cite{}.
A constraint solver consists of two main components: the \emph{modeling layer} and the
\emph{search engine}. 
Such separation between problem specification and solving algorithm allows the user to easily extend
and modify the specification without changing the solver (\textbf{C1}).
The modeling layer provides the
user with a set of expressive constraints to make the modeling process as natural as possible.
For example, it supports high-level modeling primitives like `tasks have to use disjoint resources' (\textbf{C2}).
The search engine explores the search space of the problem using techniques like constraint learning,
conflict-driven branching heuristics, etc. 
The search procedure is general, with all domain-specific knowledge encoded and passed to the solver via constraints.
Hence, constraint solvers are applicable to a wide range of optimization problems, eliminating the need to hand-craft new algorithms for each use case (\textbf{C3}).


%Next we describe each component in more detail.

\paragraph{Modeling layer}
A good modeling layer must satisfy two requirements:
in addition to facilitating the specification of complex problems, it must also capture the
high-level structure of the problem in a way that can be effectively exploited by the
search engine. This goal is achieved by exposing so-called \emph{global constraints} to the user.
A global constraint can be seen as a common pattern that occur in many problems.
One example is matching a set of objects to another set of pairwise distinct objects.
In our problem domain, such constraints can be useful to, e.g., specify that a set of pods has to be scheduled on different servers (\textbf{C2}). 
To model this pattern the \emph{all-different} constraint was introduced~\cite{}.
%Another common pattern uses finite state machines to specify rules or policies.
%This pattern is captured by the \emph{regular} global constraint that restricts assignments of a set of variables to strings in a given
%regular language\nina{Do we have an example of a rule from the MP domain for the regular constraint?}.
Constraint solvers incorporate specialized algorithms to reason about global constraints during search, discussed below.
In this work, we use MiniZinc, which is arguably the most expressive constraint modeling language available today.


%In our experiments, we compile MiniZinc into FlatZinc, the  input language of the Gecode or ORtools constraint solvers that support global constraints.
%However, there also exist compilers from MiniZinc to languages supported by SAT and ILP solvers.

\paragraph{Search} We describe the standard search procedure used by constraint solvers for finite-domain variables, since such variables are prevalent in management plane configuration problems.
\footnote{Real-valued variables are quantized in our framework. In general, Weave can support real-valued variables. However, constraint solvers that are capable of reasoning over reals and integers are less efficient compared to solvers that reason about integer variables only.}
The solver searches over the space of possible variable assignments using \emph{exploration}, \emph{inference}, and \emph{learning}.
The exploration algorithm builds the search tree of the problem, where every node represents a branching decision on one of problem variables.  The search is guided by branching heuristics.  In case of optimization problems, the cost function is used to prune the search tree and contributes to the branching heuristics.
Inference capabilities are key to the success of constraint solvers. Inference allows pruning the search space efficiently, without exploring all possible variable assignments.  This pruning is performed by so-called propagator algorithms associated with global constraints.  For example, a standard propagator for the all-different constraint uses the maximum matching algorithm to prune branches of the search tree that provably do not lead to a solution.
Often, multiple propagators for a constraint are  available in a solver. %used during search.  
Finally, learning from failures, or no-goods learning, kicks in when the
solver finds an unsatisfiable subspace of the search space.  It extracts an explanation of failure in terms of decisions that led to this subspace and uses this information to accelerate subsequent exploration.

%The search procedure is general, with all domain-specific knowledge encoded and passed to the solver via constraints.


As mentioned above, the constraint solver is a generic tool that is applicable to a wide range of optimization problems. However, it is the user's task to encode their domain knowledge using the solver's modeling constructs, as well as to configure its tunable parameters, like branching heuristics. These choices significantly impact the performance of the solver (see Section~\ref{}). As part of our system design, we analyzed a large number of MP policies and learned how to effectively make these choices in our target domain.



\lalith{The next two paragraphs are text from the HotOS submission.

We need an extended version of this.}
While notoriously hard to use for the reasons stated in
\S\ref{sec:introduction}, specialized solvers overcome the above challenges.
Solvers support input specification languages that capture complex constraints in a
modular way, even though \emph{internally}, the constraints may interact in
complex ways during the search for a solution. Therefore, developers can
easily add and modify constraints (\textbf{C1}).

The tools are capable of efficiently solving complex aggregate and global
constraints (\textbf{C2}) using techniques like bounds propagation and learning.
Lastly, these tools implement general-purpose algorithms, applicable to a wide
range of optimization problems, eliminating the need to hand-craft new
algorithms for each distributed system (\textbf{C3}). The combinatorial
optimization problems that recur across MPs are therefore best left to
specialized solvers.


We now present the basics of specialized solvers to aid the reader.


\lalith{One challenge here is to write in a common parlance across
all solvers. Not all solvers have globals for example.}

Write about:

- Propagators, global constraints

- brief summary of how the search process works

- Brief overview of solver internals that make them good
candidates to deal with challenges C1, C2 and C3.


==> sections/design.tex <==
\section{Design}
\label{sec:the_case_for_synthesis}

%As discussed in \S\ref{sec:motivation}, specialized solvers are natural
%candidates to solve the complexity challenges that MPs suffer from. However,
%solvers remain challenging to use in MP implementations, which we address in
%our design of Weave.

Weave enables programmers to specify cluster management policies in a
high-level declarative language, and compute policy-compliant configurations
automatically and efficiently. To achieve this, we have to address two design
challenges.  First, we need a specification language that is sufficiently
expressive, yet easy to use.  We chose SQL for three reasons.  First,
relational databases are already widely used to store system configuration in
existing cluster management software.  Second, unlike most formal
specification languages, SQL is familiar to most developers. Indeed, its power
has been harnessed in a wide-range of data-centric
systems~\cite{alvaro2010boom,delimitrou2015improving,cadoli2007combining}.
Finally, as we discuss in this and the following section, SQL allows
expressing complex MP policies in a clear and concise fashion.

The second challenge is to bridge the gap between the SQL representation of the problem
and formal modeling languages used by optimization tools.  To this end, we implemented
a compiler that synthesizes the necessary inputs to the solver from the SQL schema, and
a runtime engine that feeds the current state of the cluster stored in the state database
to the solver and reflects the solution returned by the solver back in the database.

As a result, Weave users do not have to learn a new language, and, more importantly,
do not have to master the subtle art of writing efficient optimization models.
%These design decisions make Weave
%unintrusive -- we leverage unmodified SQL databases, developers need not learn
%a new programming language, 
%and can incrementally add Weave to their MPs to
%solve specific sub-problems, one at a time.
%In the following sections, we
%discuss how it is like to use Weave, before describing its internals.
In the coming sections, we discuss each component in more detail.

%\nina{
%\emph{Smth along these lines I had in mind, when we discussed with Lalith this section.}
%In this section, we present the design of Weave --  a new system for cluster management tasks.
%Design of Weave is based on the principle of separation between two high-level tasks:  specifying
%cluster state and making a decision to update this state.
%Using Weave, a developer only \emph{specifies}  cluster management tasks, e.g. how to schedule pods...., in a high level language
%and the tool \emph{solves} these talks for them, e.g. finds a placement ..... .
%There are few challenges that we face here. First question is how to choose a high level language.
%We want it to be (a) expressive enough to capture rich policies in cluster management and (b) simple for developers to use.
%To this end, we make the choise of SQL language as it is a popular framework that most developers are families with.
%In fact, Weave exploits the fact that MPs today already use a database to store the cluster state and configuration. We will demonstrate below that
%it is  natural  to specify the policies on the cluster state using SQL.
%The second important question is how to find a solution to tasks specified by a developer.
%We argue that modern optimization tools should be used perform solving task.
%To use these tools, we need to bridge a gap between SQL representation of the problem and
%formal language representation of the problem that these optimization tools work with.
%Weave, transparently to a user, takes the SQL database specified by a developer
%synthesizes a low-level formal model and use a optimization solver to find a solution.
%Automatically, Weave process the solution obtained from the solver and transfers results back in the database
%ready for a developer to use. Note, that our design does not restrict us to use a particular
%optimization tool. We can plug-and-play any optimization tool as long as we have a synthesis algorithm for it.}
% \lalith{High-level goals and motivation for design is missing. Preamble mixes
% high-level description with the 'what' and 'how'.}

% Weave consists of three components: the cluster state database, the Weave
% compiler, and the Weave runtime.  The state database stores the current state of
% the cluster, e.g., ``host XXX is equipped with a GPU'', as well as end-user
% preferences, e.g., ``place pod XXX on a host with a GPU''.  It also contains SQL
% views that define the management plane policy as a set of constraints on valid
% configurations, e.g., ``for any pod XXX and host YYY, if XXX is running on YYY
% and XXX requires a GPU, then YYY must have a GPU'' (Section~\ref{}).

% At development time, the programmer uses the Weave compiler to synthesize an
% \emph{optimization model}---a program that encodes configuration constraints
% using the language of the constraint solver (Section~\ref{}).

% The Weave runtime is responsible for communication between the system and the
% solver at runtime: it initializes the solver with the optimization model
% synthesized by the compiler and populates it with data from the cluster state
% DB.  Whenever the state changes (Step~1 in Figure~\ref{fig:weave_flow}), e.g., a new pod is added to the system, Weave
% invokes the solver to compute a configuration update (Step~2), e.g., assigning the new
% pod to a suitable host while satisfying affinity constraints and optimally
% balancing load across hosts (Figure~\ref{}).  Weave converts the solution
% returned by the solver into a DB update (Steps~3 and~4).  The final step, applying the new
% configuration to the system, is implemented by the distributed system controller
% and is not part of Weave.

% We start by giving the reader an overview of how it is like to use Weave.  We
% then expand on its design and implementation in subsequent sections.

%At a high-level, to use a solver, one needs to provide a \emph{model} in a
%formal language, that describes (i) input variables supplied by the user; (ii)
%decision variables that the solver tries to identify values for; and (iii)
%constraints on the decision variables. Weave
%synthesizes this model from the database and constraints.

%, and use this model
%dynamically at runtime.
%We now describe how we derive these inputs in different steps.

\subsection{Configuration database}
\label{ssub:configuration_database}

At development time, the programmer specifies an SQL schema that represents
the cluster's state, annotating some of its columns as \emph{decision
variables}, i.e., variables to be assigned automatically by Weave. For
example, a placement decision of a pod on a node in Kubernetes can be
represented by the following:

\begin{figure}
\begin{minted}[fontsize=\footnotesize,
               frame=lines]{sql}
create table pod_info
(
  pod_name varchar(100) not null primary key,
  ....
  variable__node_name varchar(36) not null,
);
\end{minted}
\caption{A table describing pods. The \texttt{variable\_\_} prefix indicates
that the \texttt{variable\_\_node\_name} column should be treated as a set
of decision variables. Other columns are input variables, whose values are
supplied by the database.}
\end{figure}

Here, the \texttt{variable\_\_} prefix indicates that the \texttt{variable\_\_node\_name}
column should be treated as decision variables. Other columns become
\emph{input variables}, whose values are supplied by the database.

%, while other columns are treated as input variables.
%Here, the scheduler's goal is to place pods on nodes, and this decision is
%represented by the column \texttt{variable\_\_node\_name}. When Weave
%synthesizes the inputs to a solver, such columns are treated as decision
%variables, and other columns are treated as input variables.

\subsection{Policies} % (fold)
\label{ssub:policies}

The next step is to specify constraints over decision
variables. 

%We now discuss how developers specify hard constraints or soft
%constraints using SQL.

\paragraph{Hard constraints} Hard constraints are specified as SQL
views with the prefix \texttt{constraint\_}. For example, consider the
following constraint for Kubernetes:

\begin{figure}
\begin{minted}[fontsize=\footnotesize, 
               fontfamily=tt,
               frame=lines]{sql}
create view constraint_node_predicates as
select * from pod_info
join node_info 
  on pod_info.variable__node_name = node_info.name
where not(pod_info.status = 'Pending') or 
   (node_info.unschedulable = false and
    node_info.memory_pressure = false and
    node_info.disk_pressure = false and
    node_info.pid_pressure = false and
    node_info.network_unavailable = false and
    node_info.ready = true);
\end{minted}
\caption{A simple hard constraint. It ensures that pods
that are pending placement are never assigned to nodes that have been marked
unschedulable by the operator, are under resource pressure, or do not
self-report as being ready to accept new pod requests.}
\end{figure}


\begin{figure}
\begin{minted}[fontsize=\footnotesize, ,
               frame=lines]{sql}
create view constraint_node_affinity as
select *
from pods_info
where pods_info.has_requested_node_affinity = false or
      pods_info.variable__node_name in
         (select node_name
          from candidate_nodes_for_pods
          where pods_info.pod_name = 
                candidate_nodes_for_pods.pod_name);
\end{minted}
\caption{A membership constraint used to describe node affinity
requirements (the pod must only be assigned to nodes it is affine to,
as computed in another view \texttt{candidate\_nodes\_for\_pods})}
\end{figure}


\begin{figure}
\begin{minted}[fontsize=\footnotesize, 
               frame=lines]{sql}
create view demand_per_node as
select (node_info.cpu_capacity 
        - sum(pod_info.cpu_request)) as cpu_spare
from node_info 
join pod_info
  on pod_info.variable__node_name = node_info.name
where status = 'Pending'
group by node_info.name;

create view objective_least_requested_cpu as
select min(cpu_spare) from demand_per_node;
\end{minted}
\caption{A soft constraint that maximizes the minimum spare CPU capacity
in the cluster. This is used for load balancing.}
\label{fig:capacity_constraint}
\end{figure}


Here, Weave must ensure that for all records returned by joining the
\texttt{pod\_info} and \texttt{node\_info} tables, the predicate in the
\texttt{where} clause holds true. This constraint therefore ensures that pods
that are pending placement are never assigned to nodes that have been marked
unschedulable by the operator, are under resource pressure, or do not
self-report as being ready to accept new pod requests.

\paragraph{Soft constraints} Like hard constraints, soft constraints are also specified as
SQL views. However, soft constraint views need to be scalar expressions that
return a single value. Weave ensures that the computed solution
\emph{maximizes} the sum of every specified soft constraint. All views with
the prefix \texttt{objective\_} are treated as soft constraints.

As an example, consider a simple load balancing policy to balance the CPU
utilization of nodes in a cluster. To do so, we first write a convenience view
(\texttt{demand\_per\_node}) that computes the spare CPU capacity per node. We
then describe a soft constraint view (\texttt{objective\_load\_balance\_cpu})
to compute the minimum spare capacity in the cluster. By simply declaring such
a view, Weave computes solutions that maximize the minimum CPU utilization of
nodes in the cluster.

%  Weave translates these
%higher-level SQL description of the constraints into the requisite lower-level
%constraint statements as expected by a solver.

\subsection{Synthesizing optimization models}
\label{sub:synthesizing}

An optimization model expresses the optimization problem using the mathematical
formalism supported by a specific solver, e.g., a set of linear inequalities (for an ILP solver),
predicates in first-order logic (for an SMT solver), or a constraint modeling language
(for a constraint solver).

%Weave synthesizes an optimization model based on the schema and constraints.
%The schema informs Weave about input variables and decision variables in the
%model, and the constraints dictate the possible values for the decision
%variables.

By representing constraints in SQL, Weave is able to support multiple backend
languages, allowing system builders to easily try different types of solvers.
Currently, we support MiniZinc (which in turn supports a variety of solvers)
and are also implementing a backend for Google's OR-tools. With SQL being
a high-level language compared to the native interfaces of different backends,
Weave is also free to apply backend-specific optimizations during the translation
phase. We discuss these details below.

\subsubsection{Generating efficient encodings} 
\label{ssub:generating_efficient_encodings}

Solvers are highly sensitive to a problem's encoding within a model. Two
equivalent models may result in vastly different model sizes and runtimes for
the underlying solver. The Weave compiler therefore incorporates
backend-specific translations to generate efficient models for the solver to
evaluate. To motivate the need to do so, we discuss a common SQL operation:
counting the number of elements in a column that are greater than a constant.

Consider the two Minizinc statements shown in Figure~\ref{fig:minizinc}. Both
these statements compute the number of elements in an array of variables whose
value is larger than 10. In the first case, the solver cannot statically
filter the list because the values of the variables are not fixed yet. This
forces Minizinc to internally make use of \emph{optional variables}, where a
variable might be `absent' from a list. To use optional variables, MiniZinc
internally creates additional variables and constraints. For 1000 variables in
the original array, this approach creates 7001 constraints and 6001 variables
internally (Figure~\ref{fig:minizinc}). The second approach where we \emph{sum
the predicate} achieves the same result because the predicate evaluates to 0
or 1. This approach however, creates no additional constraints, and only
generates 1000 integer variables. Note that this specific approach only works
for summation. Other aggregate functions like min or max need different
optimizations.

Figure~\ref{fig:minizinc_capacity_constraint} repeats the same analysis as
Figure~\ref{fig:minizinc}, but for the more complex Minizinc code generated by
Weave for the \texttt{demand\_per\_node} view shown in
Figure~\ref{fig:capacity_constraint}. The tables represent only a hundred pods
and fifty nodes. Translating the SQL \texttt{WHERE} clause using a filter in the
constraint program produces 20.1K constraints and constraints, 5.1K
integer constraints and 15K boolean constraints. Summing the predicate instead
produces only 100 integer variables. Furthermore, the intermediate input file
generated by Minizinc for the solver is 4.4M large in the first case
(generated in 2.5 seconds) and only 4.7K in the second case (generated in
250ms).

This is one example of how Weave produces backend-specific code. It uses a
series of rules to re-write expressions depending on whether or not they can
be evaluated statically by the backend even before a solver is involved. It
applies such backend-specific transformations for different kinds of aggregate
functions. Most importantly, these are all low-level details that Weave
shields developers from when they want to use a solver to build an MP.

\begin{figure}
\begin{subfigure}{.5\textwidth}
\begin{minted}[xleftmargin=20pt,
               xrightmargin=15pt,
               fontsize=\footnotesize, 
               highlightcolor=yellow!60,
               linenos,
               label=1) sum with filter,
               highlightlines={6, 7},
               frame=lines]{text}
var int: num_values_above_ten = 
  sum([1 | i in 1..length(vars) where (vars[i] > 10)]);
\end{minted}
\label{fig:worst2}
\end{subfigure}%
\vspace{0.1in}
\begin{subfigure}{.5\textwidth}
\begin{minted}[xleftmargin=20pt,
               xrightmargin=15pt,
               fontsize=\footnotesize, 
               label=2) sum of predicate,
               highlightcolor=yellow!60,
               linenos,
               frame=lines]{text}
var int: num_values_above_ten = 
  sum([1 * (vars[i] > 10) | i in 1..length(vars)]);
\end{minted}
\end{subfigure}%
\vspace{0.1in}
\begin{subfigure}{.5\textwidth}
    % \includegraphics[width=1\linewidth, trim=0 20 0 0]{figures-arxiv/variables_created.pdf}
    % \begin{table}[ht]
\centering
\begin{tabular}{rlrr}
  \hline
 & Encoding & Vars & Constraints \\
  \hline
1 & sum with filter & 6001 & 7001 \\
  2 & sum of predicate & 1000 &   0 \\
   \hline
\end{tabular}
% \end{table}
\end{subfigure}%
\caption{Two equivalent Minizinc encodings to compute the sum over a subset
of an array of variables. The specification only has one array of a 1000 variables
and no constraints. When translated to FlatZinc however, they result
in a dramatically different number of constraints and variables for the solver.}
\label{fig:minizinc}
\end{figure}

\begin{figure}
  % \includegraphics[width=1\linewidth, trim=0 20 0 0]{figures-arxiv/variables_created_real.pdf}
  % \begin{table}[ht]
\centering
\begin{tabular}{rlrr}
  \hline
 & Encoding & Vars & Constraints \\
  \hline
1 & sum with filter & 40000 & 20100 \\
  2 & sum of predicate & 100 &   0 \\
   \hline
\end{tabular}
% \end{table}
  \caption{Number of intermediate variables and constraints generated
  by the two equivalent approaches to encoding sums shown in Figure~\ref{fig:minizinc},
  but for the \texttt{demand\_per\_node} view computed in 
  Figure~\ref{fig:capacity_constraint} (for 100 pods and 50 nodes).
  Note the log-scale for the y-axis.}
\label{fig:minizinc_capacity_constraint}
\end{figure}


\subsubsection{Re-writing expressions to use global constraints}
\label{ssub:re_writing_expressions_to_use_global_constraints}


\begin{figure}
\begin{subfigure}{.5\textwidth}
\begin{minted}[xleftmargin=20pt,
               xrightmargin=15pt,
               fontsize=\footnotesize, 
               highlightcolor=yellow!60,
               linenos,
               label=Ensure value of var is in array,
               highlightlines={6, 7},
               frame=lines]{text}
constraint forall(i in index_set(vars),
                  j in index_set(vars) where j < i) 
                  (vars[i] != vars[j]);
\end{minted}
\label{fig:worst2}
\end{subfigure}%
\vspace{0.1in}
\begin{subfigure}{.5\textwidth}
\begin{minted}[xleftmargin=20pt,
               xrightmargin=15pt,
               fontsize=\footnotesize, 
               label=Global constraint,
               highlightcolor=yellow!60,
               linenos,
               frame=lines]{text}
constraint all_different(vars);
\end{minted}
\end{subfigure}%
\vspace{0.1in}
\begin{subfigure}{.5\textwidth}
    % \includegraphics[width=1\linewidth, trim=0 20 0 0]{figures-arxiv/variables_created_alldiff.pdf}
    % \begin{table}[ht]
      \centering
      \begin{tabular}{rlrr}
        \hline
       & Encoding & Vars & Constraints \\
        \hline
      1 & With global & 101 &   2 \\
        2 & Without global & 101 & 4951 \\
         \hline
      \end{tabular}
    % \end{table}
\end{subfigure}%
\caption{Two equivalent Minizinc statements to enforce that all variables in an
 array take different values. The specification here has a 100 variables and
 a single constraint. When using a global constraint, the solver creates
 one additional variable and constraint each, whereas without using global constraints, the
 solver creates 4951 constraints.}
\label{fig:alldiff}
\end{figure}

Global constraints are constraints over \emph{groups} of variables for which
solvers implement specialized and efficient propagator algorithms that
dramatically reduce the search space of the problem. Consider for example the
common pattern of enforcing that a group of variables all take different
values. One approach is to post this constraint as a list of pairwise
inequalities (Figure~\ref{fig:alldiff}, top). The other approach is to use the
\texttt{all\_different} global constraint (Figure~\ref{fig:alldiff}, bottom).
However, for an array of 100 variables, not using a global constraint
instantiates 4950 integer constraints, whereas using a global constraint posts
only a single \texttt{all\_different} constraint, which in turn allows the
solver to use a specialized propagator.

Weave identifies opportunities to transform common SQL patterns to use a suite
of global constraints. For example, when generating MiniZinc code, we rewrite
usages of the \texttt{IN} operator in SQL and its arguments to instead use
membership global constraints for which solvers typically implement fast
propagators. Weave also allows developers to directly use global constraints
in SQL predicates. For instance, we found ourselves using the
\texttt{all\_different} constraint often to place replicas in different
failure domains, for example.

\subsection{Runtime}
\label{ssub:runtime}

At runtime, Weave is responsible for communication
between the solver and the cluster state database (Figure~\ref{fig:weave_flow}).
At startup, the solver is initialized with the optimization model synthesized
at the previous step.  Weave populates the model by extracting the values for
the input variables from the database.  Whenever the state database changes
(Step~1 in the Figure), e.g., a new pod is added to the system, Weave
invokes the solver to compute a configuration update (Step~2), e.g., assigning the new
pod to a suitable host while satisfying affinity constraints and optimally
balancing load across hosts.  Weave converts the solution
returned by the solver into a database update (Steps~3 and~4).  The final step
is to apply the new configuration to the system, which is done by the
distributed system controller and is not part of Weave.

%With the previous steps, Weave can now synthesize a constraint satisfaction
%and optimization model that can be input to a solver. What remains is to run
%this model at runtime against the changing state of the configuration
%database. Note, in practice, an MP will comprise multiple such models,
%pertaining to different functionality (e.g., one for scheduling, another for
%capacity planning, and so on).

\begin{figure}[t] \centering
    \includegraphics[width=0.5\linewidth, trim=0 30 0 0]{figures-arxiv/weave_flow.pdf}
    \caption{Weave runtime.} \label{fig:weave_flow}
\end{figure}

%\begin{table}
%\caption{Interface to the Weave library.}
%\label{tab:interface}
%{\footnotesize
%\begin{tabular}{p{3.5cm} | p{3.5cm}}
%\hline
%\texttt{1. synthesizeModel(db, policies)} & Given a connection to a relational database and a set of policies described using SQL, synthesize an optimization model. \\ \hline
%\texttt{2. updateInputs(db, model)} & Retrieve the input data for a model from the database \\ \hline
%\texttt{3. solveModel(db, model)} & Solve a model and reflect the changes in database \\ \hline
%\end{tabular}
%}
%\end{table}


\subsection{Debugging} % (fold)
\label{sub:debugging}

A common theme in debugging MPs is to understand why the MP could not identify
a valid solution (e.g., a pod placement decision) in the face of a web of
constraints.  Weave improves debuggability by taking advantage of a common
solver capability: that of identifying \emph{unsatisfiable cores}. An unsatisfiable
core is a minimal subset of model constraints and inputs that suffices to make
the overall problem unsatisfiable (for example, a core might involve a
single input variable that cannot simultaneously satisfy two contradicting
constraints in the model). We leverage this capability by providing a translation
layer that extracts an unsatisfiable core from the solver, and identifies corresponsing
SQL constraints and records in the tables that lead
to a contradiction. We found this feature invaluable when
debugging placement scenarios involving complex affinity constraints.


% subsection debugging (end)

% Given that MP architectures are architecturally similar
% (\S\ref{sub:anatomy_of_a_management_plane}) even across very different systems
% (\S\ref{tab:mps_state}), and the nature of the optimization problems they
% routinely solve are challenging to design, implement and test, we believe
% there is a strong opportunity for program synthesis. 

% Constraint satisfaction and optimization problems typically involve a
% \emph{model}, that describes input variables supplied by the user; decision
% variables that the solver tries to identify values for; and constraints on the
% decision variables. We seek to synthesize this model on behalf of the
% developer and aid in the repeated execution of this model in a solver at runtime
% against a dynamic cluster state.

% With Weave, developers architect the system to stores its cluster state as a
% collection of tables in an SQL database. Some columns in the database are
% annotated as variables (using a naming convention for columns). Weave treats
% these columns as decision variables, and other columns as input variables. The
% developer then specifies hard and soft constraints on these tables using
% standard SQL.  From the schema and the constraints, Weave synthesizes the
% required optimization model. At runtime, the model is repeatedly executed by
% drawing the values for the input variables from the database, and running it
% against a solver. Weave then reflects the output of the solver back in the
% database. The requisite programming interfaces are shown in
% Table~\ref{tab:interface}.

% \subsection{Specifying constraints using SQL views}
% \label{sub:sql_views_as_constraints}

% We now describe how developers write policies using SQL views.

% \paragraph{Hard constraints.} Hard constraints in Weave are specified as SQL
% views, which describe a selection using a predicate $p$ over a relation $r$
% (such as a table, join or sub-query expression). In relational algebra, this
% is represented as $\sigma_p\left(r\right)$, and it returns the set of records in $r$ that
% satisfy the predicate $p$. In Weave, for any hard constraint view
% $\sigma_p\left(r\right)$, Weave guarantees that the computed solutions all have
% $\sigma_p\left(r\right) = r$. That is, Weave ensures that $p$ holds true over all records
% in the relation $r$. In SQL parlance, the predicate $p$ is represented by the
% \clause{where} clause in views that do not compute aggregates, or the
% \clause{having} clause in views that do compute aggregates. Hard constraint
% views are named with a prefix \texttt{constraint\_}.

% We now show an example of such a view using a simple policy in Kubernetes.
% Nodes in Kubernetes locally report status conditions that indicate whether the
% node is experiencing resource utilization issues or whether the node is ready
% to host pods. These status conditions take the form of simple flags at each
% node, which the scheduler treats as hard constraints when it considers a node
% as a candidate to place a pod. This is represented in Weave as follows:

% \begin{minted}[fontsize=\footnotesize, 
%                fontfamily=tt,
%                frame=lines]{sql}
% create view constraint_node_predicates as
% select * from pod_info
% join node_info
%     on pod_info.variable__node_name
%        = node_info.name
% where not(pod_info.status = 'Pending') or 
%    (node_info.unschedulable = false and
%     node_info.memory_pressure = false and
%     node_info.disk_pressure = false and
%     node_info.pid_pressure = false and
%     node_info.network_unavailable = false and
%     node_info.ready = true);
% \end{minted}

% With the above constraint, Weave ensures that for all rows returned by the
% \clause{from} and \clause{join} clauses, the predicate in the \clause{where}
% clause is true. In this example, it means if a pod is waiting to be scheduled
% ({\small \texttt{status = `Pending'}}), then the status conditions of the node
% must indicate that it is schedulable, should not have any resource pressure,
% and is ready to host pods. Note, for two predicates $p$ and $q$, a clause of
% the form `not($p$) or $q$' is equivalent to a logical implication `$p$
% $\rightarrow$ $q$'.

% \paragraph{Soft constraints} To support optimization problems -- as
% opposed to only identifying solutions that satisfy all hard constraints --
% Weave also allows developers to specify soft constraints that act as objective
% functions. As with hard constraints, soft constraints are also specified as
% views, but soft constraint views need to be scalar expressions that return a
% single value. Weave ensures that the computed solution \emph{maximizes} the
% sum of every specified soft constraint. Soft constraint views are named
% with a prefix \texttt{objective\_}.

% As an example, consider a load balancing policy that maximizes the minimum
% load on each node. To do so, we first write a convenience view that computes the
% utilization of each resource (CPU, memory, storage and the number of pods).
% We then describe multiple soft constraints, written as a scalar expression each,
% to compute the minimum utilization per resource. Weave then \emph{maximizes}
% the sum of these scalar expressions.

% \begin{minted}[fontsize=\footnotesize, 
%                fontfamily=tt,
%                frame=lines]{sql}
% create view demand_per_node as
% select 
%   (node_info.cpu_allocatable 
%    - sum(pod_info.cpu_request)) as cpu_util,
%   (node_info.memory_allocatable 
%    - sum(pod_info.memory_request)) as memory_util,
%   (node_info.storage_allocatable 
%    - sum(pod_info.storage_request)) as storage_util,
%   (node_info.pods_allocatable 
%    - sum(pod_info.pods_request)) as pods_util
% from node_info
% join pod_info
%     on pod_info.variable__node_name 
%        = node_info.name
% where status = 'Pending'
% group by node_info.name;

% create view objective_least_requested_cpu as
% select min(cpu_util) 
% from demand_per_node;

% create view objective_least_requested_memory as
% select min(memory_util) 
% from demand_per_node;

% create view objective_least_requested_storage as
% select min(storage_util)
% from demand_per_node;

% create view objective_least_requested_pods as
% select min(pods_util) 
% from demand_per_node;
% \end{minted}

% \section{Synthesis}
% \label{sec:synthesis}



% Our synthesis engine produces models in a high-level, solver-independent
% modeling language called MiniZinc~\cite{minizinc}. The advantage of using
% MiniZinc



==> sections/evaluation.tex <==
\section{Evaluation} % (fold)
\label{sec:evaluation}

Our implementation of Weave is about 2K LoC in Java for the library and an
additional 1.5K LoC for tests. We first discuss our implementation of a
Kubernetes scheduler using Weave. Our scheduler works as a drop-in replacement
for the current Kubernetes scheduler (written in Go).  We evaluate both
qualitative and quantitative gains in using Weave to implement the policies in
the scheduler.

The Kubernetes scheduler has 20 configurable `predicates', which behave as hard
constraints, and 11 configurable `priorities', which are equivalent to soft
constraints. We implemented 15 of 20 predicates, where the predicates we skipped
were those that were specific to GCE, AWS and Azure. For priorities, we
implemented 4 out of 11. We are still working on implementing other
constraints, but have no reason to believe that they are any more
complicated. In general, we found ourselves spending more time studying the
existing Kubernetes code and understanding the intent behind their policies than
we did writing the equivalent code in Weave using SQL.

We were able to implement each of the constraints we considered using $<10$
lines of SQL.
%find that writing the same policies in SQL leads to fewer lines of code than
%the equivalent versions in Go.  Note, we do not include the code that the
%Kubernetes scheduler has in place to solve constraints, but only count the LoC
%used by both schemes to express policies.
We count every SQL clause (select, from, where etc.) and every predicate
separated by and/or as a new line.  For example, the \emph{service affinity}
policy, discussed in \S\ref{sec:motivation}-C2, which is challenging to get
right in Kubernetes, was implemented in only 6 lines of SQL.  It merely involves
joining one view (which itself is an additional 6 lines) and a table, and
posting a constraint using a \texttt{having} clause.  As another example, a
commonly used soft constraint in Kubernetes is the \emph{least requested}
policy, which load balances based on CPU and memory utilization.  This policy
was implemented in 4 lines of SQL -- we simply ask Weave to maximize the minimum
sum of the CPU and memory utilization per node.

%Most other constraints were even simpler that that.

%We obtained gains of between 2-4x fewer lines of code in SQL than in Go for
%predicates, and between 2.5x-12x fewer lines of code for priorities.  We found
%the improvements to be strongly correlated with the complexity of the policy: a
%simple policy that checks whether a node has a few flags enabled is as easy to
%write in Go as in SQL, whereas policies that require cross-referencing state
%across multiple data structures, or policies that constrain groups of pods/nodes
%are much harder to write in Go.
%
%thousands of lines of code tightly intertwined with its functionality and d

The number of joins is a commonly reported complexity metric for SQL.  Except
for one constraint that involved two joins, all hard and soft constraints were
expressible using zero or one joins each.

In contrast, the existing Kubernetes scheduler consists of 10s of thousands of
lines of Go code that is deeply intertwined with the rest of the system, and
is challenging to maintain and evolve.

The resulting scheduler has a performance that is competitive with the
Kubernetes scheduler. We attempt to place 400 pods on a 50 node Kubernetes
cluster. The baseline Kubernetes scheduler takes roughly 80 seconds to place all
pods. Weave on the other hand takes 35s to find an optimal solution and outputs
a near-optimal solution in only 15s.

We also implemented a management plane from scratch for CorfuDB~\cite{corfu},
a distributed transactional database. As with Kubernetes, we found it easy to
add complex features like rack-aware load balancing and flexibly partitioning
responsibilities among nodes in the cluster to be straightforward using SQL,
all of which used fewer than 10 LoC in SQL.

% \begin{table*}[t]

% \caption{Hard constraints: Lines of code comparison for Kubernetes Scheduler  
% policies written in Go vs Weave. Legend: V = number of views, S = select items, 
% W = where statements, G = group by, H = having statements, SQ = sub-queries. }

% {\footnotesize
% \begin{tabular}{| C{3cm} | C{3cm} | C{3cm} | C{1cm} | c | p{4cm} |}
% \hline
%    & Weave &  Weave  & Weave & Baseline
%    &  \\
%     Predicate & Intermediate views &  Constraint view  & Total &
%   (Go) & Description \\
% \hline
%   NodeCondition, NodeUnschedulable, CheckNodeMemoryPressurePred,
%   CheckNodeDiskPressurePred, CheckNodePIDPressurePred  & 0 & 10 
%   (W=1) &
%   10 & 19
%   &
%   Avoid nodes that report that they are not ready, are unschedulable, or are CPU, Memory, Storage or Pod over utilized. \\
% \hline
%   GeneralPred  & ? & ? &
%   ? & ?
%   &
%   PodFitsResources + PodFitsHostPorts + PodMatchNodeSelector + PodFitsHost. \\

% \hline
%   HostNamePred/PodFitsHost  & 0 & 2 (W=1) &
%   2 & 8
%   &
%   Avoid nodes that report that they are not ready, are unschedulable, or are CPU, Memory, Storage or Pod over utilized. \\
% \hline
%   PodFitsHostPortsPred  & 8 (V=1, S=4, J=1, W=1) & 8 (J=1, G=1, H=1) &
%   16 & 46
%   &
%   XXX: does not handle 0.0.0.0 case
%   \\
% \hline
%   MatchNodeSelector  & 0 & 9 (J=1, W=1, SQ=1) &
%   9 & 33
%   &
%   Avoid nodes that report that they are not ready, are unschedulable, or are CPU, Memory, Storage or Pod over utilized. \\
% \hline
%   PodFitsResources  & 9 (V=1, J=1, W=1, G=1) & 2 (W=1) &
%   11 & 38
%   &
%   XXX: does not handle scalar resources
%   \\
% \hline
%   NoVolumeZoneConflictPred  & 0 & 12 (J=1, W=1, SQ=1) &
%   12 & 54
%   &
%   XXX: does not handle unbound volumes
%   \\
% \hline
%   PodToleratesNodeTaints, PodToleratesNodeNoExecuteTaintsPred  & 0 & 12 (J=1, W=2, SQ=1) &
%   12 & 33
%   &
%   XXX: does not handle unbound volumes
%   \\
% \hline
%   CheckNodeLabelPresence  & 0 & 9 (J=1, W=1, GB=1, H=1, SQ=2) &
%   12 & 15
%   &
%   XXX: does not handle unbound volumes
%   \\
% \hline
%   ServiceAffinity  & 6 (V=1, S=1, J=1, W=1) & 5 (J=1, G=1, H=1) &
%   11 & 50
%   &
%   Services with affinitylabels are
%   placed on nodes with the same value for an affinity label \\ 
% \hline
%   MaxEBSVolumeCount, MaxGCEPDVolumeCount, MaxCSIVolumeCount,
%     MaxAzureDiskVolumeCount, CheckVolumeBinding  & TODO & TODO &
%   TODO & TODO
%   &
%   Specific to cloud platform \\ 
% \hline

% \end{tabular}
% }
% \end{table*}


% % section evaluation (end)
% \begin{table*}[t]
% \caption{Soft constraints: Lines of code comparison for Kubernetes Scheduler policies written in
% Go vs Weave}
% {\footnotesize
% \begin{tabular}{| C{3cm} | C{3cm} | C{3cm} | C{1cm} | c | p{4cm} |}
% \hline
%    & Weave &  Weave  & Weave & Baseline
%    &  \\
%     Predicate & Intermediate views &  Constraint view  & Total &
%   (Go) & Description \\
% \hline
%   SelectorSpreading  & 11 (V=1, S=2, J=2, G=1) & 1 (S=1) &
%   12 & 62
%   &
%   XXX: Weave is not incorporating zone info. \\
% \hline
%   Least Requested  & (same view as PodFitsResources) & 4 (S=4) &
%   4 & 47
%   &
%   Prioritize the lowest loaded node for each pod. \\
% \hline
%   Node Label  & 11 (V=1, S=1, J=2, W=1, G=1) & 2 (S=1) &
%   4 & 10
%   &
%   Prefer nodes that have matching labels. \\
%  \hline
% \end{tabular}
% }
% \end{table*}






==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\lalith{Lots to fix here. recheck comments from marcos and jon}
A fundamental problem in data center management is allocating resources to
 applications.  Whether juggling containers, virtual
 machines, microservices, virtual network appliances, or serverless functions,
 the \emph{management plane} must satisfy numerous resource constraints.  Some
 of these constraints are \emph{hard constraints}, which must hold in any
 valid system configuration, e.g., ``each container must obtain its minimal
 requested amount of disk space'' or ``replicas of a service must be placed on
 different server racks''. Others are \emph{soft constraints}, e.g., ``scatter
 replicas across as many racks as possible''.  Given these constraints, the
 management plane must find a configuration satisfying all hard constraints
 while minimizing violations of soft constraints.

Management plane developers usually tackle the problem by designing custom
application-specific algorithms---\emph{an approach that often leads to a
software engineering deadend}.  \nina{We need a citation here. It reads like
an unjustified claim.}As new types of constraints are introduced, the
developers get overwhelmed by having to solve arbitrary combinations of
increasingly complex constraints.  This is not surprising given that, beyond
the simplest cases, solving resource constraints amounts to an \emph{NP-hard
combinatorial problem} that cannot be efficiently solved via naive search.  In
addition to the algorithmic complexity, the lack of separation between the
application state, the policies, and the constraint solving
algorithm leads to unmaintainable code.

%Production-grade distributed systems execute a diverse range of management
%tasks, such as host lifecycle management, cluster resizing, failure recovery,
%load balancing, membership management, placement, and rolling upgrades. These
%tasks fall under the purview of a \emph{management plane} (MP) that continuously
%tracks the state of the cluster and triggers management tasks in response to
%state changes.
%
%At a high level, cluster management is guided by a set of \emph{policies} that
%represent both hard constraints ("ensure a VM requesting a GPU is always placed
%on a host with a GPU") and soft constraints ("scatter replicas across as many
%data-centers as possible").  Given a policy, the MP must find an optimal cluster
%configuration satisfying all hard constraints while minimizing violations of
%soft constraints.
%
%MP developers usually tackle the configuration problem by designing custom
%application-specific algorithms---\emph{an approach that often leads to a
%software engineering deadend}.  As new types of constraints are introduced, the
%developers get overwhelmed by having to solve arbitrary combinations of
%increasingly complex constraints.  This is not surprising given that, beyond the
%simplest cases, cluster management policies amount to \emph{NP-hard
%problems} that cannot be efficiently solved via naive
%search.  In addition to the algorithmic complexity, the lack of separation
%between the application, the policy, and the constraint solving algorithm leads
%to unmaintainable code.

We propose a radically different management plane architecture and runtime
framework, called Weave, which disentangles the application state, policies
and the solving algorithm (Figure~\ref{}).  With Weave, the developer
maintains application state in a relational database, and specifies policies
as constraints on the state using the SQL language.  At runtime, when a system
re-configuration is required, Weave combines these constraints with the
current state of the system to formulate a \emph{combinatorial optimization}
problem, which it solves using an off-the-shelf solver.  By doing so, Weave
leverages decades of progress on the solver technology, while improving the
separation of concerns in the management plane and freeing the developer from
the burden of maintaining an ad hoc solver.

%Indeed, many off-the-shelf tools exist for these problems, including constraint
%solvers, integer linear programming (ILP) toolkits, and SMT solvers. Unlike
%ad-hoc approaches, these tools enforce a separation between the specification
%of an optimization problem (the constraints) and the search algorithm used to
%solve it. These tools also incorporate decades of progress on computational
%learning, constraint propagation, symmetry breaking, and other performance
%optimizations, making them challenging to outperform with custom solutions.

%However, realizing the above vision requires us to answer the following
%question: \emph{why is the principled approach of using solvers is hardly ever
%used in production systems}?

The research community has explored the idea of solver-assisted system
configuration in various contexts, like
scheduling~\cite{Tumanov:2016:TGR:2901318.2901355,isard2009quincy}, server
provisioning~\cite{5934917}, traffic engineering~\cite{koster2010towards} and
configuration management~\cite{narain2005network}.  However this work has often
struggled to make it out of the lab due to two fundamental barriers.

%As a result, cluster management systems simply disallow many useful types of
%policies, requiring the end user to manually translate their high-level
%requirememts into low-level configuration decisions.  \leonid{Lalith, can you
%add an example here along the lines of: instead of specifying a high-level
%constraint of the form, the use must manually place the VM?}

%Our proposed MP architecture (Figure~\ref{}) separates the policy from the
%optimization algorithm implemented by the solver.  The MP developer encodes
%system configuration and policy using the solver's modeling language.  At
%runtime, the MP translates cluster state into model inputs and translates solver
%output back to a new cluster configuration (arrows in Figure~\ref{}).

%They are thus applicable to a wide range of problems, eliminating the need for
%ad hoc algorithms.

%between MP components by interposing a layer of abstraction between the system
%and the solver: the developer expresses system configuration and policy using
%the solver's modeling language, without having to worry about the details of
%the search algorithm.

%This making it easy to introduce new types of constraints, experimenting with
%different solvers,...

\paragraph{1. The adoption barrier}

Using a solver to drive cluster reconfiguration requires one to formalize
system constraints as an optimization problem, which is challenging in
practice and takes an optimization expert with an in-depth understanding of
solver internals. Importantly, this is \emph{not} a one-off effort: management
planes evolve rapidly, with new types of constraints being added on a regular
basis, and the encoding must be updated accordingly.  Modern constraint
solvers support high-level languages intended to simplify the modeling task;
however this simplicity is misleading, as naive encodings often explode in size
and yield poor performance when converted to the internal representation
used by the solver (\S\ref{sec:design}).

%In addition to the modeling complexity, solver integration involves a steep
%engineering effort in order to translate cluster state into model inputs and
%translate solver output back to a new cluster configuration at runtime.

%This complexity is hard to justify in the early days when the management plane
%only supports few constraints that can be readily solved using hand-crafted
%algorithms.  Eventually, adding new features in an ad hoc manner becomes
%infeasible.  Unfortunately, at this point the constraint solving logic is
%already intertwined with all parts of the system, making solver integration
%impossible without a major overhaul of the system (see
%Section~\ref{sec:motivation}).

\paragraph{2. The computational complexity barrier}

Clever encodings go a long way in
accelerating search for an optimal configuration.  However, the fundamental
NP-hardness of the problem kicks in eventually, as the size of the system and
the complexity of its constraints grow.  This is an important concern
in cloud-based systems, which are expected to scale elastically to very large
sizes.

%\vspace{2mm}
%
%\noindent{}Developers cope with these challenges by (1) restricting the set of
%policies users can specify, and (2) using fast best-effort search algorithms to
%find good-enough rather than optimal configurations.  As an example of the
%former, Kubernetes does not support a potentially useful constraint that limits
%the number of pods in a group hosted on the same physical node (Section~\ref{}).
%As for the latter, the Kubernetes scheduler employs a greedy search algorithm
%that schedules user workloads one pod at a time, placing each pod on the most
%suitable host before considering the next pod in the batch.
%
%Both workarounds are unsatisfactory in practice.  Restricting the set of
%supported policies hurts performance and availability, e.g., Kubernetes users
%have to either drop the pods-per-host constraint altogether, or replace it with
%an overly strict constraint that limits the number of related pods per host to
%one~\cite{}.  Likewise, best-effort search may yield configurations that make
%poor use of available hardware resources or even fail to schedule an otherwise
%schedulable workload.  These issues force users to fall back to manual placement
%(in Kubernetes, for example, clients can use affinity constraints to schedule
%pods on specific nodes), but this largely defeats the benefits of automation and
%is not sustainable at scale.

%Interestingly, both workarounds, intended to limit the complexity, often
%backfire, causing excessive complexity to be introduced down the line in order
%to oversome the limitations.  We will see examples of this in Sections~\ref{}
%and~\ref{}.

%For example, the greedy algorithm used in Kubernetes makes it hard to implement
%constraints over multiple pods, since the algorithm reasons about one pod at a
%time (Section~\ref{}).

\vspace{2mm}

%Second, management planes typically evolve from simple designs, initially only
%supporting few constraints that can be readily solved using hand-crafted
%algorithms.  At this stage, the complexity of integrating a solver into the
%system is hard to justify.  By the time the developers hit a brick wall, where
%adding new features in an ad hoc manner becomes infeasible, the system has
%accumulated too much technical debt, with constraint solving logic being deeply
%intertwined with all parts of the system.  At this point, integrating a solver
%in the system requires its major overhaul, which rarely happens in practice (see
%Section~\ref{sec:motivation} for an example).

%However, today's management planes are not built in a principled way that allow
%the above-mentioned constraints to be easily defined and solved in a sound and
%efficient manner. Instead, they are built as large monolithic programs written
%using imperative programming languages, where the cluster state and policies
%are coupled with one another. This has several negative implications: it makes
%testing system behavior challenging, it is difficult to reason about the
%guarantees the system provides, it limits the pace at which features can be
%added and evolved over time, and it makes it challenging to evaluate how
%external events might cause the system to react ("how many VMs will be migrated
%if rack X fails?").

%However, there exist advanced formal tools for solving sets of constraints,
%like constraint solvers, SMT solvers and LP solvers. While these tools are a
%natural fit for solving the kind of constraint-satisfaction problems that
%management planes tackle, they are unfortunately not straightforward to use.
%They expect as input both an abstract model of the problem in a formal language
%(constants, variables, constraints and objective functions), and the data
%forthe model (values for the constants) -- a drastically different approach
%than how today's management planes are developed. Constraint programming
%frameworks also lack standardized languages, frameworks and ecosystems that
%developers can lean on. In addition, there is the added complexity of
%repeatedly computing and applying solutions computed by the solver against a
%dynamic system where the state is continuously evolving.  Finally, encoding a
%problem efficiently into a constraint program involves a steep engineering
%effort, effort that recurs every time developers set out to build each new
%system.

\subsection*{Design principles}
To tackle the above mentioned challenges, Weave's design is based on three key principles.:
\begin{itemize}
    \item Re-use existing languages and tooling used by developers
    \item Hide solver complexity 
    \item Exploit the incremental nature of cluster management
\end{itemize}


\subsection*{Our approach}
\label{sub:our_approach}
\nina{The first sentence reads like the main purpose of Weave is  to squeeze a solver in management plane. I think it is more general than that.
Perhaps, smth like: Weave presents a new approach to \emph{automating solver-based system
configuration}.}
Weave eliminates the above barriers by \emph{automating solver-based system
configuration}.  Weave exploits the fact that in modern distributed systems
the information required to formulate and solve the configuration problem is
readily available in the \emph{cluster state database}.  This database
maintains an up-to-date view of cluster configuration, including its physical
inventory, workload, and user preferences.  Instead of requiring the
developer to build a separate system model for use by the solver, Weave
extracts this model from the database schema.

\nina{The flow is not  smooth in the next three paragraphs.
They describe two modes of operation but we never mention this explicitly.}
Weave programmers express hard and soft constraints (or the policy) as a
collection of SQL views over the state database.  Thus, they do not need to learn the
low-level language of the solver, and instead work with familiar SQL.

Given the state database schema extended with views, Weave generates an
efficient encoding of the configuration problem in the constraint solver's
language.  It uses the high-level information extracted from SQL to generate
optimized encodings that would be hard for non-expert users to hand-craft
(Section~\ref{}).

At runtime, Weave automates the communication between the MP and the solver by
extracting current cluster configuration from the state database and converting
it into an input to the solver.  It parses the solution computed by the solver
and outputs the requisite modifications (deltas) to be made to the database state
to satisfy all the policies. A controller, written by the developer, converts
these deltas into lower-level control plane commands to the underlying
system.

Weave overcomes the computational complexity barrier by leveraging the
incremental nature of cluster management: in a production cluster, the workload
and the physical topology change gradually over time. The MP responds to changes
by making incremental updates to cluster configuration, e.g., scheduling new
tasks on the least loaded hosts, often without touching existing workloads.
From the optimization perspective, \emph{restricting the scope of changes the MP
can perform during reconfiguration dramatically shrinks the search space to be
explored by the solver.}

This observation informs the design of the Weave \emph{incremental optimization
framework}.  Weave searches for a new configuration within a user-defined target
search scope.  At one extreme, the user may request a global optimum, possibly
finding a new resource allocation for all workloads in the system.  At the other
extreme, Weave schedules one unit of work, e.g., a single task, at a
time.  While both extremes are available in Weave, they are seldom used.

%, thus degenerating to the greedy search used in today's cluster managers.

%This is typically neither computationally feasible, nor practically useful, as
%rearranging all workloads can be highly disruptive.

\lalith{The below paragraph seems to suggest that the tool is smart enough to
figure out what corresponds to "components directly affected by the event". It isn't.
It's just that Weave lets developers seamlessly control the degree of incrementalness
in the models.}
In practice, developers using Weave use one or more intermediate options.
In a typical setup, Weave responds to external events by searching for an optimal reconfiguration of only
those components directly affected by the event, e.g., when the user submits a
workload consisting of a group of tasks, Weave tries to optimally place the new
tasks without relocating any of the existing ones.  If the resulting
optimization problem is too hard to solve within a time budget, Weave breaks up
the workload into smaller batches and schedules them one-by-one.  If, on the
other hand, Weave discovers that the new workload is not schedulable in the
current configuration, it relaxes the problem and searches for an optimal
placement that involves relocating up to a configurable number $n$ of existing
tasks.  By restricting the search space in this way, Weave is able to schedule
incoming jobs in real time, within a few seconds (Section~\ref{}).

In addition, Weave can be configured to perform cluster-wide optimization at a
larger time scale.  For example, given a larger time budget of a few minutes Weave can
compute a configuration that reschedules up to $N$ tasks in order to improve
resource utilization across the cluster (Section~\ref{}).

%Crucially, Weave does all of this without requiring any extra input from the
%developer.  It automatically generates different encodings of the SQL
%constraints


%With Weave, developers represent the cluster configuration in an SQL database
%as a collection of relations.  They express hard and soft constraints (or the
%policy) on that state as a collection of SQL views.  Given this information,
%the Weave library \emph{synthesizes a combinatorial optimization program},
%solves it using an off-the-shelf constraint solver, and outputs the requisite
%modifications (deltas) to be made to the database state to satisfy all the
%policies. A controller, written by the developer, observes these deltas and
%issues lower-level control plane commands to the underlying system.

%Weave completely or partially automates ...:
%
%\begin{itemize}
%
%    \item \emph{System modeling}: Weave eliminates the need to develop a
%        separate formal model of the system for use by the solver.  Instead, it
%        automatically extracts the model from existing system configuration
%        database.
%
%    \item \emph{Policy specification}:
%
%        it simplifies modeling of the relational model.  so that the developer
%        does not have to work with the low-level modeling language of the
%        underlying solver.
%
%(2) Efficiency: Weave generates an
%
%high-level constraints.
%
%Optimizations, e.g., incremental solving, ...
%
%switch between backend solvers, encoding styles.
%
%(3) Integration:
%
%\lalith{The advantages we discussed: - Opportunity for optimizations  (global constraints, incremental changes, local vs global search)
%- solver independence
%- debugging with unsat cores
%- higher-level representation of constraints for programmability
%- ease of integration: just add constraints on top of existing data models. At runtime, automate the process of the loop.
%}

%Weave's design poses three advantages. First, developers already use SQL
%databases to store cluster state and are familiar with the SQL language, which 
%is standardized. Second, the use of SQL allows Weave to augment existing 
%management plane implementations and not require a complete re-write of the 
%code base using a constraint-programming toolkit. Third, the separation of 
%state and policy required by Weave simplifies automated testing and running 
%what-if scenarios.

% We used Weave to implement a Kubernetes scheduler, and management planes
% for CorfuDB and Redis Cluster. We achieved code size reductions of XXX, and
% managed to easily add complicated features like rack-aware load balancing etc.
% The resulting system is still fast, capable of making management plane 
% decisions in a system with a BAJILLION nodes and a QUINTILLION pods, in
% sub-second timescales. This paper will describe these efforts, and end with
% challenges that remain to be addressed.


==> sections/introduction2.tex <==

\section{Introduction} 
\label{sec:introduction}

Management planes (MPs) are a critical component of any production-grade
distributed system. The MP continuously tracks the state of the cluster and
performs myriad management tasks like host lifecycle management, cluster
resizing, failure recovery, load balancing, membership management, placement,
and rolling upgrades. The MP carries out these tasks to conform to several
operator- and user-defined policies; these policies may represent hard
constraints (``do not exceed the resource utilization limits of a machine''),
and soft constraints (``spread replicas across as many availability zones as
possible''). In doing so, MPs routinely juggle hard combinatorial optimization
problems, making them challenging to design, develop, test and evolve over
time.

Unfortunately, developers tasked with building MPs for production-grade
systems are faced with two poor options.

The most common approach used to build today's production MPs, is to develop
ad-hoc mechanisms per-system to solve these optimization problems, often using
conventional programming languages. Beyond the simplest cases, this approach
soon hits a steep complexity wall because of the NP-hard nature of common
cluster management tasks; as the system evolves and new types of constraints
are introduced, developers get overwhelmed by having to solve arbitrary
combinations of increasingly complex constraints.

The second approach is to leverage specialized solvers. Many off-the-shelf
tools exist for solving combinatorial optimization problems, including
constraint solvers, integer linear programming (ILP) toolkits, and SMT
solvers. \lalith{would skip this line}These tools incorporate decades of
progress on computational learning, constraint propagation, symmetry breaking,
and other performance optimizations. Indeed, researchers have explored
solver-based distributed system management in the context of
scheduling~\cite{Tumanov:2016:TGR:2901318.2901355,isard2009quincy}, server
provisioning~\cite{5934917}, traffic engineering~\cite{koster2010towards} and
configuration management~\cite{narain2005network}.

However, \emph{the principled approach of using solvers is hardly ever used in
production systems.} This is because of three key practical obstacles.
\textbf{(C1)} First, hand-crafting an efficient optimization model to solve a
system's constraints requires an optimization expert who is familiar with a
solver's internals. Naive and often natural encodings often yield poor performance,
even for small problem sizes. Furthermore, this engineering cost of crafting an encoding is not a
one-off effort: MPs evolve rapidly, with new types of constraints being added
regularly, and the encoding must be updated accordingly. \textbf{(C2)} Second,
solver interfaces are not standardized, making it challenging to switch seamlessly
between them. This introduces a significant amount of risk for
developers to adopt a solver within an existing code base. \textbf{(C3)} Third,
even specialized solvers eventually run into the fundamental NP-hardness of
the problems being solved, a challenge exacerbated in large distributed
systems where the state space is potentially large. In the absence of a
principled way to bound runtimes, developers are wary of using a solver in a
large system.

This paper presents Weave, a tool that eliminates the above barriers by
\emph{automating solver-based system configuration}. Weave makes it easy for
developers to use solvers to tackle hard management plane problems, without
the three aforementioned engineering obstacles that using a solver typically
entails.

Weave exploits the fact that in modern distributed systems the information
required to formulate and solve the configuration problem is readily available
in a \emph{cluster state database}. This database maintains an up-to-date view
of cluster configuration, including its physical inventory, workload, user
preferences, etc.  Instead of requiring the developer to build a separate
system model for use by the solver, Weave extracts this model from the
database schema (\textbf{C1}).

Weave programmers express hard and soft constraints (or the policy) as a
collection of views over the state database.  Thus, they do not need to learn the
low-level language of the solver, and instead work with familiar SQL (\textbf{C2}).

Given the state database schema extended with views, Weave generates an
efficient encoding of the configuration problem in the constraint solver's
language.  It uses the high-level information extracted from SQL to generate
optimized encodings that would be hard for non-expert users to hand-craft
(Section~\ref{})  (\textbf{C1}).

At runtime, Weave automates the communication between the MP and the solver by
extracting current cluster configuration from the state database and converting
it into an input to the solver.  It parses the solution computed by the solver
and outputs the requisite modifications (deltas) to be made to the database state
to satisfy all the policies. A controller, written by the developer, observes
these deltas and issues lower-level control plane commands to the underlying
system.

Weave overcomes the computational complexity barrier by leveraging the
incremental nature of cluster management: in a production cluster, the workload
and the physical topology change gradually over time. The MP responds to changes
by making incremental updates to cluster configuration, e.g., scheduling new
tasks on the least loaded hosts, often without touching existing workloads.
From the optimization perspective, \emph{restricting the scope of changes the MP
can perform during reconfiguration dramatically shrinks the search space to be
explored by the solver} (\textbf{C3}).

This observation informs the design of the Weave \emph{incremental optimization
framework}.  Weave searches for a new configuration within a user-defined target
search scope.  At one extreme, the user may request a global optimum, possibly
finding a new resource allocation for all workloads in the system.  At the other
extreme, Weave schedules one unit of work, e.g., a single task, at a
time.  While both extremes are available in Weave, they are seldom used.

In practice, developers using Weave use one or more intermediate options.
In a typical setup, Weave responds to external events by searching for an optimal reconfiguration of only
those components directly affected by the event, e.g., when the user submits a
workload consisting of a group of tasks, Weave tries to optimally place the new
tasks without relocating any of the existing ones.  If the resulting
optimization problem is too hard to solve within a time budget, Weave breaks up
the workload into smaller batches and schedules them one-by-one.  If, on the
other hand, Weave discovers that the new workload is not schedulable in the
current configuration, it relaxes the problem and searches for an optimal
placement that involves relocating up to a configurable number $n$ of existing
tasks.  By restricting the search space in this way, Weave is able to schedule
incoming jobs in real time, within a few seconds (Section~\ref{}).

In addition, Weave can be configured to perform cluster-wide optimization at a
larger time scale.  For example, given a larger time budget of a few minutes Weave can
compute a configuration that reschedules up to $N$ tasks in order to improve
resource utilization across the cluster (Section~\ref{}).


==> sections/introduction3.tex <==

\section{Introduction} 
\label{sec:introduction}

Management planes (MPs) are a critical component of any production-grade
distributed system. The MP continuously tracks the state of the cluster and
performs myriad management tasks like host lifecycle management, cluster
resizing, failure recovery, load balancing, membership management, placement,
and rolling upgrades. The MP carries out these tasks to conform to several
operator- and user-defined policies; these policies may represent hard
constraints (``do not exceed the resource utilization limits of a machine''),
and soft constraints (``spread replicas across as many availability zones as
possible''). In doing so, MPs routinely juggle hard combinatorial optimization
problems, making them challenging to design, develop, test and evolve over
time.

Unfortunately, developers tasked with building MPs for production-grade
systems are faced with two poor options.

The most common approach used to build today's production MPs, is to develop
ad-hoc mechanisms per-system to solve these optimization problems, often using
conventional programming languages. Beyond the simplest cases, this approach
soon hits a steep complexity wall because of the NP-hard nature of common
cluster management tasks; as the system evolves and new types of constraints
are introduced, developers get overwhelmed by having to solve arbitrary
combinations of increasingly complex constraints.

The second approach is to leverage specialized solvers. Many off-the-shelf
tools exist for solving combinatorial optimization problems, including
constraint solvers, integer linear programming (ILP) toolkits, and SMT
solvers. \lalith{would skip this line}These tools incorporate decades of
progress on computational learning, constraint propagation, symmetry breaking,
and other performance optimizations. Indeed, researchers have explored
solver-based distributed system management in the context of
scheduling~\cite{Tumanov:2016:TGR:2901318.2901355,isard2009quincy}, server
provisioning~\cite{5934917}, traffic engineering~\cite{koster2010towards} and
configuration management~\cite{narain2005network}.

However, \emph{the principled approach of using solvers is hardly ever used in
production systems.} This is because of three key practical obstacles.
\textbf{(C1)} First, hand-crafting an efficient optimization model to solve a
system's constraints requires an optimization expert who is familiar with a
solver's internals. Naive and often natural encodings often yield poor performance,
even for small problem sizes. Furthermore, this engineering cost of crafting an encoding is not a
one-off effort: MPs evolve rapidly, with new types of constraints being added
regularly, and the encoding must be updated accordingly. \textbf{(C2)} Second,
solver interfaces are not standardized, making it challenging to switch seamlessly
between them. This introduces a significant amount of risk for
developers to adopt a solver within an existing code base. \textbf{(C3)} Third,
even specialized solvers eventually run into the fundamental NP-hardness of
the problems being solved, a challenge exacerbated in large distributed
systems where the state space is potentially large. In the absence of a
principled way to bound runtimes, developers are wary of using a solver in a
large system.

This paper presents Weave, a tool that eliminates the above barriers by
\emph{automating solver-based system configuration}. Weave makes it easy for
developers to use solvers to tackle hard management plane problems, without
the three aforementioned engineering obstacles that using a solver typically
entails.

Weave exploits the fact that in modern distributed systems the information
required to formulate and solve the configuration problem is readily available
in a \emph{cluster state database}. This database maintains an up-to-date view
of cluster configuration, including its physical inventory, workload, user
preferences, etc.  Instead of requiring the developer to build a separate
system model for use by the solver, Weave extracts this model from the
database schema (\textbf{C1}).

Weave programmers express hard and soft constraints (or the policy) as a
collection of views over the state database.  Thus, they do not need to learn the
low-level language of the solver, and instead work with familiar SQL (\textbf{C2}).

Given the state database schema extended with views, Weave generates an
efficient encoding of the configuration problem in the constraint solver's
language.  It uses the high-level information extracted from SQL to generate
optimized encodings that would be hard for non-expert users to hand-craft
(Section~\ref{})  (\textbf{C1}).

At runtime, Weave automates the communication between the MP and the solver by
extracting current cluster configuration from the state database and converting
it into an input to the solver.  It parses the solution computed by the solver
and outputs the requisite modifications (deltas) to be made to the database state
to satisfy all the policies. A controller, written by the developer, observes
these deltas and issues lower-level control plane commands to the underlying
system.

Weave overcomes the computational complexity barrier by leveraging the
incremental nature of cluster management: in a production cluster, the workload
and the physical topology change gradually over time. The MP responds to changes
by making incremental updates to cluster configuration, e.g., scheduling new
tasks on the least loaded hosts, often without touching existing workloads.
From the optimization perspective, \emph{restricting the scope of changes the MP
can perform during reconfiguration dramatically shrinks the search space to be
explored by the solver} (\textbf{C3}).

This observation informs the design of the Weave \emph{incremental optimization
framework}.  Weave searches for a new configuration within a user-defined target
search scope.  At one extreme, the user may request a global optimum, possibly
finding a new resource allocation for all workloads in the system.  At the other
extreme, Weave schedules one unit of work, e.g., a single task, at a
time.  While both extremes are available in Weave, they are seldom used.

In practice, developers using Weave use one or more intermediate options.
In a typical setup, Weave responds to external events by searching for an optimal reconfiguration of only
those components directly affected by the event, e.g., when the user submits a
workload consisting of a group of tasks, Weave tries to optimally place the new
tasks without relocating any of the existing ones.  If the resulting
optimization problem is too hard to solve within a time budget, Weave breaks up
the workload into smaller batches and schedules them one-by-one.  If, on the
other hand, Weave discovers that the new workload is not schedulable in the
current configuration, it relaxes the problem and searches for an optimal
placement that involves relocating up to a configurable number $n$ of existing
tasks.  By restricting the search space in this way, Weave is able to schedule
incoming jobs in real time, within a few seconds (Section~\ref{}).

In addition, Weave can be configured to perform cluster-wide optimization at a
larger time scale.  For example, given a larger time budget of a few minutes Weave can
compute a configuration that reschedules up to $N$ tasks in order to improve
resource utilization across the cluster (Section~\ref{}).


==> sections/motivation.tex <==
\section{Motivation} % (fold)
\label{sec:motivation}

\leonid{The plan is to remove this section altogether (after checking that all the useful bits appear elsewhere).}

\begin{table}
\caption{MPs cluster state and policy examples across systems.}
\label{tab:mps_state}
{\footnotesize
\begin{tabular}{| l | p{2.5cm} | p{3cm} |}
\hline
\textbf{System} & \textbf{Example cluster state} & \textbf{Example policies} \\ \hline
Kubernetes & Pods, nodes, volumes, labels, ports, services & Affinity rules, availability zone constraints, resource utilization, load balancing \\ \hline
OpenStack & VMs, nodes, volumes, disks, networks & Affinity rules, availability zone constraints, resource utilization, load balancing \\ \hline
HDFS & nodes, files, directories, inodes, blocks, permissions & rack-awareness, replication rules, load balancing \\ \hline
\end{tabular}
}
\end{table}

Although the exact functions of the management plane vary across systems, at a
high level they all share a common MP architecture, consisting of three key
components: a model of the cluster state that describes the configuration of
the distributed system, a policy (or constraints) that the cluster should
conform to, and a control loop that ensures that the cluster state always
conforms to the policy. We present examples of cluster states and policies
across different systems in Table~\ref{tab:mps_state}.
We now consider the two main approaches for MPs to specify and solve
constraints.

\subsection{Status quo: ad-hoc mechanisms}
\label{ssec:ad_hoc_mechanisms}

Today's MPs typically use ad-hoc mechanisms to specify constraints and solve
them. This is because distributed system management planes often start small
and humble. For example, version~1 of the system may rely exclusively on the
user to configure the system manually. As the frequency and complexity of
management tasks increase, some automation is introduced, including support
for simple policies and a naive search algorithm. Eventually, more complex
constraints are added to enable large-scale deployment scenarios. Before long,
developers find themselves grappling with three major challenges:

\begin{description}
 \item [C1] Adding new types of constraints is hard, because they interact in complex
  ways with existing constraints, often requiring completely or partially
  reimplementing the search algorithm when new constraints are
  introduced.

 \item [C2] Search strategies become suboptimal or inefficient, especially in the
 face of \emph{global constraints} (e.g., constraints that hold over
 entire groups of VMs). \lalith{Mention optimizations. Use references from
 Firmament paper about caching, pre-computing etc.}

 \item [C3] The constraints and search algorithm become tightly coupled with the
  application-specific policies and state, hindering re-use of these
  mechanisms across projects. For example, the algorithm used to place VMs in OpenStack
  cannot be re-purposed to schedule containers in Kubernetes.
\end{description}

\subsection{Motivating example: Kubernetes scheduler}
\label{sub:motivating_example_kubernetes}

We use the \emph{Kubernetes scheduler}~\cite{kubernetes} to illustrate the limitations of the
ad-hoc approach to cluster management. However, the challenges associated with
the ad-hoc approach are general and recur across different MPs, not just
Kubernetes.

The scheduler is responsible for assigning
collections of containers, called \emph{pods}, to cluster nodes.
In the current implementation it works as follows:
For each pending pod placement request, the scheduler first iterates through
each node in the system, and filters out the set of valid nodes using a list
of \emph{predicates} (analogous to hard constraints). The scheduler ranks all
the valid nodes using some priority functions (analogous to soft constraints).
The pod is finally placed on the highest ranked node.

This design is simple, flexible (allowing developers to contribute new
predicates and priority functions), and efficient.  Unfortunately, it also
proved fundamentally limited when it comes to expressing more complex
constraints due to three main challenges discussed above.

%The above architecture allows developers to contribute new predicates and
%priority functions in a modular way. However, this architecture has
%fundamental limitations when it comes to expressing more complex policies. We
%will focus on examples for the three challenges discussed above that arise
%because Kubernetes does not have a systematic way of specifying constraints
%and solving them against its cluster state.


\paragraph{Dependencies among constraints (C1)} Some time after the basic
scheduling algorithm was implemented, Kubernetes introduced a new
\emph{eviction} policy: if the scheduler cannot place a pod, it checks whether
it can preempt existing lower priority pods.  This policy interacts with the
basic node placement policy: the preemption code verifies whether
affinity/anti-affinity predicates for the original pod were in use, and if they
will be violated if that lower priority pod is evicted (causing those predicates
to be re-executed).

As new, more complex predicates are added, the preemption code needs to remain
in sync with the rest of the scheduler, making it challenging to evolve the
code over time.  The complexity accumulates making entire classes of policies
difficult to implement in the scheduler. For example, cross-node preemption,
where a pod on one node is preempted to allow a new pod to be placed on
another node (because of affinity/anti-affinity requirements) is currently not
possible~\cite{crossnodepreemption}.

\paragraph{Global constraints (C2)} Consider Kubernetes' \emph{service affinity}
predicate. The predicate ensures that all pods from the same service (e.g., a
fleet of load balancers) are assigned to nodes that have identical values for
some configured labels (e.g., an availability zone label). This constraint
holds over \emph{groups} of pods and nodes, but it is hard to implement this
in the current scheduler architecture that can only reason about placing pods,
\emph{one at a time}. Therefore, the scheduler, when placing each pod from a
group, has to scan some data-structures to make sure its next decision will be
consistent with past decisions for pods from the same service. The scheduler
therefore contains additional code to pre-compute some of these results to
avoid the inefficient scans.

Not surprisingly, the code is commented with a large warning that indicates
that the predicate is not guaranteed to work without the precomputed metadata,
and there is a discussion to ax the feature because of the accumulating
technical debt~\cite{serviceAffinityHard}. Similarly, the global nature of
affinity/anti-affinity policies too have raised discussions among developers
to remove the feature (or simplify what users are allowed to do to make the
code efficient)~\cite{podAffinityHard}. This challenge is aggravated by the
fact that a series of caching and pre-computing optimizations used to speed-up
policies like inter-pod affinity/anti-affinity are hard to maintain when
requirements evolve (for example, to extend these policies to specify the
number of pods per node~\cite{podTopologyCount1,
podTopologyCount2,podTopologyCount3,podTopologyCount4,podTopologyCount5}).

\paragraph{Coupling between policies and state (C3)} Finally, all the scheduler code
is tightly coupled with the data-structures that hold the cluster state. For example,
it is not possible to re-use the code for defining constraints and
solving them in Kubernetes to be used in a different system. This is inherent
in not just the interfaces to add new predicates and priorities, but also in
 all the associated code of the scheduler around preemption.


% \paragraph{\textbf{Specialized solvers}}
% While notoriously hard to use for the reasons stated in
% \S\ref{sec:introduction}, specialized solvers overcome the above challenges.
% Solvers support input specification languages that capture complex constraints in a
% modular way, even though \emph{internally}, the constraints may interact in
% complex ways during the search for a solution. Therefore, developers can
% easily add and modify constraints (\textbf{C1}).

% The tools are capable of efficiently solving complex aggregate and global
% constraints (\textbf{C2}) using techniques like bounds propagation and learning.
% Lastly, these tools implement general-purpose algorithms, applicable to a wide
% range of optimization problems, eliminating the need to hand-craft new
% algorithms for each distributed system (\textbf{C3}). The combinatorial
% optimization problems that recur across MPs are therefore best left to
% specialized solvers.


% section approach (end)

% Hard to test, application specific, no code reuse, infrequently triggered on
% live systems and therefore may have a lot of bugs hiding.

% Some anecdotal evidence on this front:
% - vSAN: 100s of policies, takes 4-6 releases (multiple years) to add and
%   stabilize new features

% - Kubernetes: 40 policies, they interact in subtle ways.

% - hand wave: huge search space, integration testing is hard as there are many
%   moving parts

% Management planes 


% XXXXXXXXXXXXXXX:
% motivation has two parts. One, why are these things difficult to develop.
% Actually, systems are more similar than they seem even though domain is different.

% And then two, so why is it possible to have something generic.


==> sections/motivation2.tex <==
\section{Motivation} % (fold)
\label{sec:motivation}


\section{Problem statement}
\label{sec:problem_statement}




\subsection{Building management planes is challenging}
\label{sec:building_management_planes_is_challenging}

Building robust management planes is challenging because they they lack a
systematic way of specifying and solving complex sets of constraints. Instead,
they are typically built using ad-hoc mechanisms written using imperative
programming languages. These mechanisms typically take the form of greedy
heuristics to identify the desired state of a cluster, along with some checks
to enforce hard constraints. 

\paragraph{Problem 1: Aggregate constraints}
First, the predicates and priorities cannot easily specify
invariants on the
cluster in aggregate: if a developer wants to write a predicate that needs to
hold against a group of pods, or a group of nodes, the code begins
accumulating technical debt (give examples -- selector spreading, nominated
pods etc. --- podFitsHost being run twice).

\paragraph{Problem 2: Constraints with mutual dependencies}
Second, the approach works poorly if predicates have mutual dependencies. For
example, affinity/anti-affinity constraints have subtle interactions with the
scheduler's decision making around preemption. Therefore, the preemption code
needs to identify decisions made in a different part of the code base (namely,
when the scheduler first attempted to pack a pod), to decide whether a node
should be a candidate for a preemption, and if so, which pod in it should be
picked. Similarly, when identifying lower priority pods to remove, the
preemption code needs to verify whether there are affinity/anti-affinity
constraints for the original pod that will be violated if that lower priority
pod is evicted. In a similar vein, Kubernetes cannot support cross-node
preemption, where a pod on a node X is preempted to allow a pod to be placed
on node Y (such that a global resource or affinity/anti-affinity constraint is
satisfied). These are all symptoms of a more basic problem: the lack of a
mechanism to clearly compose constraints that have mutual dependencies.

\paragraph{Problem 3: Lack of guarantees}
Lastly, it is unclear what guarantees and invariants the code is trying to
preserve as a whole. Consider the discussion in this PR, where the developers
are trying to carefully document the intent of the code because the imperative
code written in Go focuses on the how. This is a problem that can be addressed
using declarative approaches where the intent is directly specified, but how
to achieve it is left to a specialized tool like a compiler or a solver.

\subsection{Management planes as a constraint satisfaction problem}
\label{sub:management_planes_as_a_constraint_satisfaction_problem}


To illustrate these issues, we turn to
Kubernetes, a widely used container orchestration platform. The problems we
discuss below are by no means unique to Kubernetes, and in fact we believe
Kubernetes is one of the better engineered systems we have seen over the
course of this study.

In Kubernetes, when users request pods to be scheduled, the scheduler first
iterates through each node in the system, sequentially checks whether a list
of predicates (hard constraints) can be satisfied against that node, and then
proceeds to rank all the node using some priority functions (soft
constraints). The pod is finally placed on the highest ranked node. This
architecture allows developers to contribute new predicates and priority
functions in a modular way. However, this architecture has fundamental
limitations when it comes to expressing more complex policies. We will focus
on three problems that arise because Kubernetes does not have a systematic way
of specifying constraints and solving them against its cluster state.

